Solving a Flowshop Scheduling Problem with Answer Set Programming: Exploiting the Problem to Reduce the Number of Combinations

Planning and scheduling have been a central theme of research in computer science. In particular, the simplicity of the theoretical approach of a no-wait flowshop scheduling problem does not allow to perceive the problem complexity at first sight. In this paper the applicability of the Answer Set Programming language is explored for the solution of the Automated Wet-etching scheduling problem in Semiconductor Manufacturing Systems. A method based in ranges is proposed in order to reduce the huge number of combinations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{347}
\providecommand{\publicationstatus}{B. Bogaerts, E. Erdem, P. Fodor, A. Formisano,\\ 
G. Ianni, D. Inclezan, G. Vidal, A. Villanueva, \\
M. De Vos, F. Yang (Eds.): International \\
Conference on Logic Programming 2019 (ICLP'19).\\
EPTCS 306, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.306.41}{10.4204/EPTCS.306.41}}
\pdfoutput=1

